When does Bias Transfer in Transfer Learning?

Using transfer learning to adapt a pre-trained "source model" to a downstream "target task" can dramatically increase performance with seemingly no downside. In this work, we demonstrate that there can exist a downside after all: bias transfer, or the tendency for biases of the source model to persist even after adapting the model to the target class. Through a combination of synthetic and natural experiments, we show that bias transfer both (a) arises in realistic settings (such as when pre-training on ImageNet or other standard datasets) and (b) can occur even when the target dataset is explicitly de-biased. As transfer-learned models are increasingly deployed in the real world, our work highlights the importance of understanding the limitations of pre-trained source models. Code is available at https://github.com/MadryLab/bias-transfer

==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}




\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/old/intro.tex <==
Transfer learning is a machine learning paradigm
% in which one first trains on a {\em source task} (e.g.,
% classifying Imagenet images), then adapts the resulting model to a second {\em
in which one uses data from a {\em source dataset} (e.g., ImageNet) 
to solve a second {\em target task} (e.g. classifying a different dataset, or
detecting objects). 
% The goal is to obtain models that are more performant on the target task than
% ones trained from scratch on the target dataset.
In image classification, a typical transfer learning pipeline comprises two
steps: {\em training} a model on the source task, and {\em adapting} the
trained model to fit the target data.


Generally, prior work has found that the richer and larger the source dataset,
the more performant the final model will be across a wide variety of downstream
target tasks.
As a result, {\em large pre-trained models} are
% (i.e., ones trained on massive, often proprietary datasets) 
a compelling starting point from
which to adapt to target tasks. 

These models, however, can have a variety of hidden biases, from poor
performance on underrepresented subgroups to dependence on spurious correlations.
% Biases often stem from patterns or subpopulations in the training
% data---
% but 
Furthermore, when transfer learning from a pre-trained model, downstream
practitioners have no access to the source dataset, from which such biases often
originate.
A natural question---and the one we focus on in this work---is thus:
\begin{center}
{\em In transfer learning, to what extent do biases in source datasets 
leak into models' behavior on target tasks?}
\end{center}
In particular, 

% In this work, we examine this question in detail.
Our starting point is an affirmative answer to perhaps the most basic form of
the question, studied by \citet{gu2017badnets}. 
Specifically, the authors consider the case where an adversary {\em poisons} the
source dataset by introducing a backdoor attack (that is, a ). 
\citet{gu2017badnets} show that if one trains a neural network on the poisoned 
dataset, then adapts the last layer of the network to an (unpoisoned) target
task, the resulting model will still be vulnerable to the backdoor attack.



- Perhaps the most basic form of this question has been answered in the
affirmative by \citet{gu2017badnets} and others \citep{TODO}. Specifically, they
show that if an attacker plants a {\em backdoor} (a spurious feature ... ), 
then models transferred from the backdoored model will also be backdoored
- But, [backdoors are the most extreme type of spurious correlation] and
[usually totally not present in the soruce task] and [last layer only].





% Deep neural networks currently achieve state-of-the-art performance across many
% computer vision tasks. These models are trained from scratch when large quantities of labeled data and computing resources are available. However, in many practical settings there is insufficient data or compute for this approach to be viable. 
% In such cases, {\em transfer learning}~\citep{donahue2014decaf, razavian2014cnn}
% has emerged as a simple and efficient way to obtain performant models. Transfer
% learning refers to any machine learning algorithm that leverages information
% from one (``source'') task to better solve another (``target'') task. In
% practice, people often use public off-the-shelf pretrained models or datasets. 
% However, no attention is paid to the biases or the vulnerability that these pretrained models or datasets might have. Thus, an important question that we ask is:

\begin{center}
    \textit{If the source task includes biases (and the target task do not), do these biases show up in the transferred model?}
\end{center}

\paragraph{Our contributions.}
In this work, we find that although target datasets in transfer learning might
not include biases, the resultant model could be biased due to inherent biases
transferred from the source task. 
We characterize the extent to which such biases transfer via extensive
experiments studying the effect of model size, strength of bias, transfer
technique, etc. on a suite of image classification tasks. We further demonstrate
that biases transfer in more realistic scenarios such as object detection,
facial recognition, and medical classification tasks. 
Our findings suggest that more caution should be taken when transferring
knowledge from large open-source datasets or pre-trained models---even in the
case where the target task is clean/curated---to avoid transferring undesired
biases to the downstream tasks. 


% Machine learning models frequently pick up biases and vulnerabilities from the
% data they are trained on.
% These biases manifest in ways ranging from performing poorly on underrepresented
% subgroups \citep{TODO}, to depending on spurious correlations \citep{TODO},
% to learning unintended input-label associations \citep{TODO}.
% In many cases, we can trace biases back to specific patterns or
% subpopulations in the dataset---making access to data imperative for 


% Transfer learning is a paradigm for training machine learning models
% in which one first trains a model on a {\em source task} (e.g.,
% classifying Imagenet images), then adapts the model to a second {\em target
% task} (e.g. classifying a different dataset, or detecting objects).

- At this point, we know that neural networks pick up on biases in the data
- To counter this, we need to audit bla bla bla, doing so has surfaced many
biases, very good
- But, an emerging paradigm in ML is transfer learning, where one .. 
- Pre-trained models attractive for this purpose

- But: pre-trained models are by design trained on large, often proprietary
datasets
- No matter how much we clean up and work with the target data, we can't do
anything about the source data.
- This raises the importance of the question:

[ Bla bla bla ]


- 

